What Will 5G Be?

What will 5G be? What it will not be is an incremental advance on 4G. The previous four generations of cellular technology have each been a major paradigm shift that has broken backwards compatibility. And indeed, 5G will need to be a paradigm shift that includes very high carrier frequencies with massive bandwidths, extreme base station and device densities and unprecedented numbers of antennas. But unlike the previous four generations, it will also be highly integrative: tying any new 5G air interface and spectrum together with LTE and WiFi to provide universal high-rate coverage and a seamless user experience. To support this, the core network will also have to reach unprecedented levels of flexibility and intelligence, spectrum regulation will need to be rethought and improved, and energy and cost efficiencies will become even more critical considerations. This paper discusses all of these topics, identifying key challenges for future research and preliminary 5G standardization activities, while providing a comprehensive overview of the current literature, and in particular of the papers appearing in this special issue.

==> control.tex <==
\subsection{Latency and Control Signaling (Volunteer?)}

JA: I have latency and control signaling grouped together but they could be separated possibly.  There is some close coupling for sure though as the latency requirements mainly impact the control channels (resource request, assignment and allocation, etc.)    Also, having a dense mmWave-based small cell network with massive MIMO has very serious implications on the control channels, that need discussion.  However, we could also discuss each of their implications above instead.  For example, ``soft cells" and the need for beam acquisition and tracking for mmWave; orthogonalization of control channels and pilots in the context of heavily biased small cells, plus the difficulty in supporting mobility in a very dense environment; and the training nightmare/pilot contamination for a massive MIMO system with non-trivial mobility, especially at high carrier frequencies (bigger doppler).


SB: Another point is the advent and explosion of machine-to-machine communications. many predict that in coming years billions of devices (cars, washing machines, heaters, meters, etc...) will be wirelessly connected. While these devices usually have few bits to send on air, the problem is that the signaling overhead in LTE does not depend on the amount of data to be transmitted, so it might happen that the network ends up overwhelmed by signaling messages originated for the transmission of very small messages. There is a paper produced by the 5GNOW european project wherein it is shown that the signaling traffic is growing much faster than the payload traffic. This is a problem that is related mainly to higher layers of the communication stack, so I do not know if we have to talk a little bit about it or neglect it...\\

==> standards.tex <==

\section{Standardization and Economic Challenges (2 pages)}

\subsection{5G Regulation and Standards (CZ and AS)}
\label{sec-standards}

5G has gained a lot of attention in the last couple years, and several regional forums and projects were established to provide a vision for 5G and to study the key 5G enabling technologies~\cite{ITU-METIS, ChinaPromotion,Arib,5GKorea }. For example, the EU Mobile and Wireless communications Enablers for the Twenty Twenty Information Society has initiated work on the requirements for 5G mobile system, and has published documents on  scenarios, requirements and KPIs,  as well as  potential technology~\cite{METIS12013,METIS22013}. Meanwhile,  5G has been increasingly referred to as ``IMT-2020'' in many industry forums and ITU  working group discussions, e.g.~\cite{ITU-R2014-1}. The goal is to achieve commercial deployment of 5G networks starting from year 2020, as the name suggests.  To achieve this goal,   ITU-R working party 5D has set a target to complete a vision document as a draft new recommendation to ITU-R by June 2015. This vision document, titled ``Framework and overall objectives of the future development of IMT for 2020 and beyond'', is to help generate momentum and accelerate global research, technology development, and standardization activities, with a goal of successful launch of 5G systems around year 2020.

The issue of new spectrum for mobile communication has also received significant attention at the ITU. ITU WP5D~\cite{ITU-R2014-2} has been actively studying the feasibility of  higher-frequency bands ($>6$GHz) around many technical aspects, including channel modeling, semiconductor readiness, coverage, mobility support, as well as potential deployment scenarios and coexistence with existing cellular networks.  The motivation is straightforward: if we can make use of %these
high frequency spectrum that is relatively abundant, %at higher frequencies,
then much of  the spectrum shortage we are experiencing today can be alleviated. This will encourage continued innovation and investment in the wireless space,  and further improve the mobile computing experience for billions of users around the world, as discussed in Section~\ref{sec-spectrum}.  The semiconductor industry has made major progress on mmWave technology  in the last decade, and mmWave wireless solutions and products are now available in the 60GHz band for high-rate, short distance communications (known as WiGiG devices),  in the 28 and 38 GHz for fixed wireless communications,  and  in the E-band (71-76, 81-86 GHz) for wireless backhauling.  GaAs MMIC (Monolithic Microwave Integrated Circuit) is improving fast and is expected to be mature enough in the next few years to provide commercial-grade power-efficient PA, LNA, VCOs, phase shifters and necessarily other RFIC solutions.

For mmWave mobile communications to be ready for 5G, the relevant spectrum has to be re-purposed by national regulatory bodies for mobile purposes, and further agreed in ITU WRC (World Radiocommunication Conferences) as global bands for mobile communications. These processes tend to be tedious and lengthy, and there are many hurdles to clear before these spectrum bands can be ready for commercial mobile deployments.  On the ITU side, it is all but certain that in the upcoming WRC-15 meeting the focus of discussion will be on $<6$GHz bands only as a first step to relieve the critical shortage of spectrum for the industry. The second step at WRC-18 is viewed by many in the industry as the right time and venue to agree on higher frequency spectrum bands for future IMT mobile systems. In fact, recently several proposals  were submitted to EU regional WRC preparation meetings, with the goal of getting higher frequency spectrum for future IMT agreed in WRC-18.   In addition to these ITU activities, many national regulatory bodies have also started their own studies on using mmWave band for mobile communications. For example, in U.S. the   FCC's technology arm TAC (Technological Advisory Council) has carried out extensive investigation on mmWave technology in the last few years, and it is possible that FCC will issue an NOI (Notice of Inquiry) about mmWave band in 2014, which is the first step in FCC's rulemaking process for allocation of any frequency bands.

The actual 5G standardization has not formally started in 3GPP, the main standard body for cellular communications technologies. To explore the user requirements driving 5G and start to elaborate the standards agenda driven by them, ETSI on November 23, 2013 held a Future Mobile Summit~\cite{Scrase}. The Summit concluded that evolution may not be sufficient to meet the anticipated 5G requirements, and that 3GPP methodology may need to be revisited for 5G standardization. 3GPP is currently finishing up LTE Release 12, which is the third release for its LTE-Advanced family of standards.  The timing of 5G standardization has not been agreed upon but it is not expected to start until a later release such as Rel-14 or 15, likely to be around the time of year 2016 or 2017. On the other hand, many ongoing and proposed study items in Rel-12 is closely related to several 5G candidate technology mentioned in this paper. For example, the FD-MIMO (Full-Dimension MIMO) technology discussed earlier in this paper was presented in a recent proposal~\cite{RP-140273}, as a follow-up study for the ongoing 3D channel modeling effort in 3GPP Rel-12.  Meanwhile, several other recent proposals bring new thoughts and ideas to how spectrum is used in the future for mobile communications. For example, licensed-band spectrum sharing was proposed in~\cite{RP-140158}, while a method of extending LTE to unlicensed bands (also known as LTE-U) was proposed in~\cite{RP-140260}.


\subsection{Economic issues (SH,  CZ?) }
\label{sec:economics}

%This section does not include spectrum issues which are already discussed.

Here, we need some sort of introductory paragraph to move from the spectrum regulation above to the economics of sharing below.

\subsubsection{New economic models for 5G networks}

In recent years, there has been a transition from voice-centric to data-centric networks. Traffic volume %, in bits carried,
and revenue have decoupled, with revenue per bit falling rapidly, whilst demand for data has been exploding. Economic theory predicts that carriers will invest in more capacity to meet the growing demand, but falling revenues are limiting the opportunity for capacity growth.

Market theory predicts that prices go up if demand increases and supply is limited. Indeed, unlimited data plans were partly responsible for the explosive growth in demand, and now that carriers are moving toward tiered data plans, there are signs that the growth rate is slowing to better match supply \cite{Budde2013}. Nevertheless, the goal of the regulator is to maximize social welfare, {\it i.e.} to increase carried traffic at lower prices to the consumer, but with enough profit-making incentives for investment in infrastructure. This is an economic problem and one that may require new business models.

As we have discussed, the most effective way to increase supply is for carriers to invest in small-cell networks, to get the most re-use of radio spectrum. New approaches to spectrum regulation will lower barriers to entry, increasing small-cell capacity. One approach is to make spectrum free, although we have seen in Section~\ref{sec-spectrum} that this doesn't always work, and careful modeling is required. Another approach is to ensure that spectrum is efficiently shared amongst multiple providers. If the latter, the providers do not need to pay as much in spectrum license fees as under the exclusive license model. These issues were discussed in Section~\ref{sec-spectrum}.

Even if spectrum costs can be reduced, it remains a challenge for carriers to implement small-cells. Base station sites are expensive and so is the backhaul needed to connect them together. Small-cell data traffic is much more bursty which implies that utilization will be lower.

A new business model that appearing recently addresses these issues. In this model, the owners of infrastructure and the service providers are different. This enables many different carriers to use the same network of base stations. For example, in the USA there are aggregators, such as Crown Castle and American Tower, who have deployed (or bought) base station sites, which they then lease to multiple service providers.

The sharing of infrastructure can be passive or active. Passive elements of a network are base station towers or sites (physical space, rooftops, towers, masts and pylons), cable, power supply, air-conditioning {\it etc}. Operators can cover a larger geographical area at lower cost if they agree to share towers or sites, and this will be particularly important in 5G networks which require dense networks of base stations. Site sharing can also reduce power consumption and improve the environment (less towers) and improve competition \cite{MRG11}. However, regulation may be required to ensure that new entrants to 5G are not disadvantaged by 4G operators who already have pre-exisitng 4G sites. Regulation may require large networks to share their sites with other operators to improve competition.

Active infrastructure sharing includes antenna sharing, base station sharing, radio access network sharing and even core network sharing. This type of sharing can lead to collusion, with anti-competitive agreements on prices and services \cite{MRG11}. Regulations may be required to prevent such collusion. However, such sharing provides economies of scale. Antenna sharing may be required in spectrum sharing scenarios, since antennas will be optimized for certain bands.

Base station and/or radio access network sharing may be very attractive when rolling out networks of small cells \cite{GMW13}. If the pico-cell radio access network is shared by several service providers (SPs), the pico base station has access to each SP's frequency allocations, but each customer is restricted to their SP's band. If the core network is shared, then the pico-cell may be able to pool frequencies, and allocate them more efficiently. 

A small cell may be owned by virtual mobile network operator (MVNO) who does not own any spectrum. This MVNO may enter a roaming agreement with a SP to get access to that SP's spectrum in the small cell. The small cell may provide coverage of an enterprise or business. When a customer leaves the enterprise it then roams onto the SP's network. Alternatively, the MVNO may have spectrum and offer service across a network of small cells, covering various enterprises. It enters into roaming agreements with multiple service providers to provide outdoor coverage across a wide area \cite{GMW13}.

Roaming is the traditional way for SP's to share their networks. Roaming is used to increase coverage in scenarios when each SP's geographical reach is limited. However, in 5G, roaming may be very useful to manage capacity, since traffic fluctuations will be much greater in small-cell networks. On the other hand, such agreements may limit the incentive of each SP to invest in infrastructure {\it eg.} small-cell base stations.

A recent paper, \cite{BHNSZV13}, investigates the incentive for investment under various revenue-sharing contracts. The model consists of two SPs, and SP $i$ receives a revenue of $p_i$ per unit demand that it carries, and incurs a cost $c_i$ per unit of capacity that it provides, $i = 1, 2$. In \cite{BHNSZV13}, the capacity is ``spectrum'', but it can just as easily be infrastructure, such as the number of small cells. The demand, $D_i$, is unknown, but the distribution is known. If the SPs don't share capacity, then the two problems are independent, each a version of the classic newsvendor model. If there is no sharing then the optimal investment can easily be found. Spare capacity exists for SP $i$ if $D_i < c_i$. In \cite{BHNSZV13}, two sharing models are considered. In the first, the SP will serve its own customers first, and if it has any spare capacity, it will carry the other SP's overflow traffic (if any) for a fee. In the second model, the SP's do not discriminate between their own users and those of the other carrier. In both models, a parameter ($\alpha$ or $\beta$, both in $[0,1]$) determines how much of the revenue goes to one carrier or the other, in the case when overflow traffic is carried.

The interaction between the carriers is modeled as a game, in which the SPs invest in such a way to maximize their individual expected profit under the given sharing rule. It is shown that sharing increases investment, and the incentive is greater if the owner of the infrastructure gets the larger fraction of the revenue when overflow traffic is carried. 

Another work to consider sharing of capacity between two providers is \cite{LMK14}. In this work, energy consumption is the main consideration: Each SP must decide whether or not to switch on their base station. If SP A switches on its base station, it incurs an energy cost, but it also receives a payment for carrying SP B's traffic. If A's base station is switched off, A must pay B to carry A's traffic. In either case, there is a penalty for not serving all one's own traffic. A game-theoretic approach is taken, in which each SP makes selfish decisions. The main focus of the paper is on the existence and characteristics of the Nash equilibria.

\subsubsection{Other issues???}

\begin{itemize}
\item Will providers be willing to do a full on 5G upgrade or instead want incremental improvements to LTE, more WiFi, etc?  See other discussion in this section.

\item Will providers put other economic incentives in place that have a major effect on how these networks function or what they must do?  E.g. moving from unlimited to tiered data plans very substantially slowed the data explosion growth rate in just a couple years.  (See Cisco VNI report for data on this).

\item Backhaul could go here as well as this is a major challenge for both densification (more miles of ``pipes'') and mmWave or any other rate-increasing technology (need a much thicker ``pipe'').

\item Small cell deployments aren't currently very economic in many cases because cities and other entities are insisting on a similar cost structure (i.e. very large monthly rental fees) and permitting process as used for macrocells.  This is a huge challenge to meeting our vision for densification, which otherwise is ready for action.

%\item SH: High cost of infrastructure, and high variability of demand (cf small cells), naturally leads to sharing of base stations/backhaul/spectrum, this requires a new economics of wireless networks, and new methods of regulation.   JA agrees, increasingly in the USA aggregators like Crown Castle and American Tower buy out or create the BS sites and then lease them out to whoever wants them (i.e multiple service providers), creating new efficiencies in terms of infrastructure sharing.  Not sure how it works in Europe or Asia but its a sensible business model for 5G BS deployment it seems to me.

\item Could some new disruptive force, e.g. Facebook or a startup, create a huge network of semi-open access WiFi APs?  For example, you allow others to learn your password and get access and in return you get access to theirs?  Some start ups are definitely trying to do this, but none have critical mass to really make a difference.  I bet a lot of people who do this if it was simple and resulted in them getting tons of newly available WiFi APs to roam on, especially in the new world of tiered data plans. AL: Perhaps the most successful example of this is FON (www.fon.com) already running over 12 million hotspots.

\end{itemize}

